A Variance-Decomposition Formula for Direct and Adjoint Monte Carlo Particle Transport Problems

In fixed-source Monte Carlo particle-transport problems, obtaining an acceptable variance on the sought response is of paramount importance. Currently, the only rigorous tool to analyze the variance of such games is the framework of the moment equations, which is unfortunately unwieldy to use in practice. In this paper, we establish a formula that enables expressing the variance of a Monte Carlo simulation as a sum of 'variance contributions' collected throughout the underlying particletransport process. This formula applies to both direct and adjoint games, and provides a new tool to pinpoint the variance-inducing mechanisms in Monte Carlo simulations, understand common variance-reduction techniques, and even conceive new ones. We showcase the use of the variance-decomposition formula on several applications. In particular, we revisit zero-variance schemes and analyze existing variance-reduction techniques, underlining their strengths and weaknesses. A few relevant numerical examples substantiate our theoretical findings.

==> Content/Multi_part.tex <==
\section{UNUSED: Multi particles}

\subsubsection{Multi-particle population control}
\label{sec:multi_part_pop_control}

Now, let us focus on multi-particle population control. The details of how to adapt the variance-decomposition formula for the specific samplings involving several particles is treated in \cref{sec:multi_part_process}. The problem of single-particle population control such as roulette or splitting appears when the average number of offsprings that we want to create is not an integer (see \cref{eq:var_pop_control}), since in this case some random selection process is mandatory. Collectively acting on a collection of particles allows for finer control, while still creating an integer number of offsprings. For instance, suppose that we want to reduce the population by a factor of $2/3$; in this case, we can apply combing to groups of $3$ particles to reduce them to $2$ particles. If $3$ particles are found at the same point $P$ of phase space, this is doable without having to use a stochastic process, and this process adds no variance. If a different factor is sought, we can apply the procedure to a large number of particles to get arbitrarily close to the sought factor, and thus generate arbitrarily small variance. 

The obvious problem is that, except if we are simulating a discrete phase space, the probability of finding any number of particles at the exact same point $P$ is null. To circumvent this issue, we can apply population control on particles at different points in phase space. This procedure, however, requires to choose which particles will survive (or will be split). Since the different entering positions will have a different importance, the importance of the outcome (which is the collective importance of all the particles produced by the combing) will depend on the choice of particles done in combing even if the number of outgoing particles is a fixed integer (and variance is thus generated).

An ideal solution to this dilemma would be to increase the number of particles in the simulation, so that population control can be applied only on particles that are found close to each other. Increasing the number of particles, the distance in phase space of the different particles upon which combing will be applied decreases, and this in turn decreases the difference in importance of the different particles. If all the entering particles have increasingly similar importance, the importance of the different outcomes of the combing also get increasingly similar, and this mechanically decreases the variance of the combing process. In the limit of arbitrarily many particles, one can apply combing to particles arbitrarily close, with arbitrarily close importance, and thus with arbitrarily small induced variance. This is how we can ideally adapt the sampling intensity at will all over phase space without generating extra variance; this is needed in the FoM-optimal strategy described in \cref{sec:fomtimal_solutions}.



==> Content/Non_independent_source_particles.tex <==
\section{Non-independent source particles}
\label{sec:non_indep_source_part}
In this section, we will specifically treat the question of non-independent source particles. Although a situation of non-independence of the source particles might seem far-fetched, any procedure that affects the particles collectively can affect the independence of the particles. The most widely used example is population combing, that is used over the whole population to obtain a given number of particles. Combing is e.g.~used in time-dependent Monte Carlo simulations in the context of reactor physics in order to adjust the number of neutrons and precursors (See for example Refs.~\citet{sjenitzer_dynamic_2013,faucher_new_2018,montecchio_adaptive_2025}. Such a procedure impacts particles collectively, and correlates the stories of different particles (the survival probability of one particle is affected by the number of the other particles), and voids the independence hypothesis that is customarily adopted to justify the convergence of Monte-Carlo games.

Let us first derive a pathological configuration breaking the independence in a way that will prevent any convergence of the Monte Carlo game towards the expected value when the number of source particles is increased. This extreme case, presented in \cref{fig:pathological_non_independent_example}, relies on a combing procedure applied on the whole population in order to reduce the number of particles to a fixed number $N^*$ that does not depend on the number of source particles $N$. Using this procedure, even if the number of source particles is arbitrarily increased, the number of subsequent offsprings will remain fixed to $N^*$, and all the remaining sampling operations will add variance that will not decrease. For those samplings, the relative contribution $c_r(P)$ is left unchanged as $N$ grows. However, since the particle density $n(P)$ is unchanged (because of the combing to a fixed number of offsprings), the relative number of particles $n(P)/N$ decreases, leading to $I_s(P)$ scaling as $N^{-1}$ (see \cref{eq:sampling_intensity}). In the variance-decomposition formula (\cref{eq:decomp_var}), this decrease of $I_s(P)$ will cancel out the $1/N$ term, preventing the sought convergence.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/Pathological_Non_independent.pdf}
    \caption{Example of a `pathological' Monte-Carlo game that breaks the hypothesis of independence of source particles. This game simulates the $N$ source particles up to a given point, and then reduces the number of particles to a fixed number $N^*$ that does not scale with $N$, before resuming the simulation. This game is unbiased, but will not converge to the expected value as $N$ grows.}
    \label{fig:pathological_non_independent_example}
\end{figure}

Of course, the scheme presented in \cref{fig:pathological_non_independent_example} fails precisely because we prevented the number of particles from increasing, using combing. If one uses combing with a target number of particles that is kept proportional to $N$, the convergence will occur at the expected speed. This cannot be proven using the hypothesis of independence of the source particles (as they are not strictly independent, due to combing); yet, it can be proven using the variance-decomposition formula \cref{eq:decomp_var}. According to the formula, the specific sampling that corresponds to the combing operation decreases proportionally to $N$. The proof of this statement relies \cref{eq:decomp_var_multi_part_sampling}; its (quite cumbersome) derivation is left for future work. The remaining terms corresponding to the other samplings will have their number of particles $n(P)$ scale proportionally to $N$, so that $n_r(P)$ will remain unchanged, and the whole sum remains unchanged. Therefore, the $1/N$ term guarantees the sought convergence speed.

==> Content/Zero_variance_estimators.tex <==
\section{Zero-variance estimators}
\label{sec:zv_estimators}

In \cref{sec:zero_variance}, we examined a fixed-source problem where zero-variance was achieved by altering the source, flight and collision sampling, and adjusting the weights accordingly; the estimator was not modified. In this section we will find a partially-unbiased estimator that enables zero-variance, for a given set of sampling laws. This result can be also achieved using the moment equations; an example is provided in Chap.~5, Part VIII of Ref.~\citet{lux_monte_2018}. The fact that the estimator is partially-unbiased means that the associated result $R$ will converge towards the same sought response $\esp{R}$. In order to obtain a zero-variance game, we still have to satisfy \cref{eq:zv_implication}. However, instead of changing the sampling rules to modify the weight multipliers $m_k$, this time we will modify the estimator function to adapt the value of $M_1$.

In order to keep $M_1(X_P)=\sum_{k=1}^K m_k M_1(P\to P'_k)$ constant, we can score using the modified estimator:
\begin{equation}
   h_{zv}(P,P'_k)=\frac{M_1(P)}{Km_k}-M_1(P'_k),
   \label{eq:zero-variance_estimator}
\end{equation}
with $K$ being the number of sub-particles being produced. The importance $M_1(P\to P')$ can be expressed as a sum of the estimator functions $h_{zv}(P\to P'_k)$, plus the final importance $M_1(P'_k)$. The sum is then:
\begin{equation}
    \sum_{k=1}^K m_kM_1(P\to P'_k) = \sum_{k=1}^K m_k \left[ \frac{M_1(P)}{Km_k}-M_1(P'_k) + M_1(P'_k) \right] = M_1(P).
\end{equation}
This expression only depends on the entering point $P$, and is thus constant for all outcomes of the current sampling. This formula will fail if either $K=0$ (there exists an outcome where no particles are being produced), or $m_k=0$ (there exists an outcome where the weight of the particle is multiplied by zero). This stems from the assumptions of scoring with the outgoing weight of the particle: if the particle does not exist, or if $m_k$ is zero, we cannot score the appropriate amount. We can circumvent this issue by assuming that any absorption, leakage or multiplication by zero of the weight actually sends the particle to the death state $P_\text{death}$, which has zero importance, i.e. $M_1(P_\text{death})=0$. In this case, we score $M_1(P)$.

For $h_{zv}(P,P'_k)$ to properly work, the estimator needs to be sensitive to the number $K$ of outgoing particles, and to the weight multipliers $m_k$. This means that such kind of estimator is different for each reaction type, and is aware of any weight-modifying scheme such as implicit absorption or branchless collisions. For the total game to be zero-variance, this estimator needs to be used at every sampling, including the sampling of the source. This requires to score $M_1(P_\text{source})-M_1(P')$ when a particle is sampled at point $P'$, where we introduced the state $P_\text{source}$ that represents the particle before its birth is sampled. The importance of a particle in that state is directly the sought response $\esp{R}$. Finally, one needs to have perfect knowledge of $M_1$ at all points,  including $P_\text{source}$, i.e.~ we need to know $\esp{R}$ exactly. If we try to use an approximation of $M_1$, for example from a deterministic calculation, the obtained result will be biased. 

The constraint that the estimator should be partially unbiased means that the expectation of the score over a cycle of flight plus collision should be the same as the expectation of the score from the `natural' response function $\eta_\psi$ (see \cref{eq:partially_unbiased_direct} and more generally Chap.~5 part VI of Ref.~\citet{lux_monte_2018}). We are then free to choose how we score within a flight and collision cycle, but the first moment $M_1$ at emission points $P$ must be equal to $\chi^\dagger(\mathcal{P})$. This means that there exist different possibilities of distributing the estimator function over the cycle. In the case of an analog, non-multiplying game, where we can score $h_t(\mathcal{P},\mathcal{P}')$ during flights and $h_c(\mathcal{P}',\mathcal{P}'')$ during collisions\footnote{As in \cref{eq:partially_unbiased_direct}, we use the convention that in the case of absorption or leakage the operators send the particle to $P_\text{death}$, which ensures that the operators are normalized and the particles can score when leaking or being absorbed.}, we could use:
\begin{align}
    h_t(\mathcal{P},\mathcal{P}')&=M_1(P) - M_1(P')\\
    h_c(\mathcal{P}',\mathcal{P}'') &= M_1(P')-M_1(P'').
\end{align}
Alternatively, the estimator can be global, i.e. 
\begin{align}
    h_t(\mathcal{P},\mathcal{P}')&=M_1(P) \\
    h_c(\mathcal{P}',\mathcal{P}'') &= -M_1(P'').
\end{align}
In either case, at the end of the cycle from point $P$ to point $P''$, the particle has scored $M_1(P)-M_1(P'') = \chi^\dagger(\mathcal{P})-\chi^\dagger(\mathcal{P}'')$, and the adjoint transport equation yields
\begin{align}
&\chi^\dagger(\mathcal{P}) = \int T(\mathcal{P}\to \mathcal{P}') \eta_\psi(\mathcal{P}')d\mathcal{P}' + \int T(\mathcal{P}\to \mathcal{P}')\int C(\mathcal{P}'\to \mathcal{P}'')\chi^\dagger(\mathcal{P}'') d\mathcal{P}''d\mathcal{P}'\nonumber\\
\Leftrightarrow& \int T(\mathcal{P}\to \mathcal{P}')\eta_\psi(\mathcal{P}')d\mathcal{P}' = \int T(\mathcal{P}\to \mathcal{P}')\int C(\mathcal{P}'\to \mathcal{P}'') (\chi^\dagger(\mathcal{P})-\chi^\dagger(\mathcal{P}''))d\mathcal{P}''d\mathcal{P}'\nonumber\\
\Leftrightarrow& \int T(\mathcal{P}\to \mathcal{P}')\eta_\psi(\mathcal{P}')d\mathcal{P}' = \int T(\mathcal{P}\to \mathcal{P}')\int C(\mathcal{P}'\to \mathcal{P}'') (h_t(\mathcal{P},\mathcal{P}')+h_c(\mathcal{P}',\mathcal{P}''))d\mathcal{P}''d\mathcal{P}'.
\label{eq:proof_partially_unbiased_zv}
\end{align}
\Cref{eq:proof_partially_unbiased_zv} ensures that the estimator satisfies \cref{eq:partially_unbiased_direct} and is indeed partially unbiased.

An intuitive explanation of how this estimator works in the case of non-multiplying analog games is that a particle, along its history consisting of points $P_i$, will score:
\begin{equation}
    R_\text{curr} = \frac{1}{N}\sum_i h(P_{i-1},P_i) = \frac{1}{N}\sum_i M_1(P_{i-1})-M_1(P_i) = \frac{M_1(P_0)}{N} = \frac{M_1(P_\text{source})}{N} = \frac{\esp{R}}{N},
\end{equation}
where we used the fact that the last point of the series is $P_\text{death}$, whose importance is 0. 

Finally, observe that the definition of the zero-variance estimator in \cref{eq:zero-variance_estimator} might lead to negative scoring, if the importance of an outgoing point $M_1(P'_k)$ is larger than $M_1(P)/(K m_k)$. This is contrary to the hypothesis of the `positive' Monte-Carlo game. However, in the formal proof in \cref{sec:proof}, we show that we only need the hypothesis $M_1\ge0$ for the formula to be valid. As long as the original game was `positive' (verifying $M_1\ge0$) the modified zero-variance game will still have $M_1  \ge 0$, and the variance decomposition formula \cref{eq:decomp_var} holds true.
